Binary Black-box Evasion Attacks Against Deep Learning-based Static Malware Detectors with Adversarial Byte-Level Language Model

Anti-malware engines are the first line of defense against malicious software. While widely used, feature engineering-based anti-malware engines are vulnerable to unseen (zero-day) attacks. Recently, deep learning-based static anti-malware detectors have achieved success in identifying unseen attacks without requiring feature engineering and dynamic analysis. However, these detectors are susceptible to malware variants with slight perturbations, known as adversarial examples. Generating effective adversarial examples is useful to reveal the vulnerabilities of such systems. Current methods for launching such attacks require accessing either the specifications of the targeted anti-malware model, the confidence score of the anti-malware response, or dynamic malware analysis, which are either unrealistic or expensive. We propose MalRNN, a novel deep learning-based approach to automatically generate evasive malware variants without any of these restrictions. Our approach features an adversarial example generation process, which learns a language model via a generative sequence-to-sequence recurrent neural network to augment malware binaries. MalRNN effectively evades three recent deep learning-based malware detectors and outperforms current benchmark methods. Findings from applying our MalRNN on a real dataset with eight malware categories are discussed.

==> am_engine_table.tex <==
\begin{tabularx}{1\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\raggedright\arraybackslash}X 
  | >{\raggedright\arraybackslash}X | }
 \hline
 Anti-Malware Engine & Owner & Reference \\ [0.5ex] 
 \hline
 MalConv & Laboratory for Physical Sciences & Raff et al., 2018 \\ 
 \hline
 NonNeg & Laboratory for Physical Sciences & Flashman et al., 2019\\
 \hline
 ConvNet & Avast & Krcal et al., 2018 \\
 \hline
\end{tabularx}

==> append_volume_table.tex <==
\begin{table}[h]
\caption{Evasion rates and number of required training iterations obtained at different append sizes}
\small
\begin{tabularx}{0.5\textwidth} { 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X | }
 \hline
 \textbf{AVG Append Size (\%)} & \textbf{AVG Append Size (KB)} & \textbf{\# of Evaded Samples} & \textbf{Evasion Rate} & \textbf{\# of Training Iterations} \\
 \hline
 5 & 7.5 & 763 & 82.4\% & 14,357\\
 \hline
 10 & 15 & 862 & 93.09\% & 8,588\\
 \hline
 20 & 30 & 882 & 95.25\% & 5,133\\
 \hline
 40 & 66 & 906 & 97.84\% & 3,169\\
 \hline
 80 & 132.8 & 910 & 98.27\% & 3,065\\
 \hline
 100 & 166 & 912 & 98.49\% & 3,205\\
 \hline
 120 & 199.2 & 919 & 99.24\% & 2,840\\
 \hline
 180 & 298.8 & 921 & 99.46\% & 2,406\\
 \hline
\end{tabularx}
\label{append_volume}
\end{table}

==> benchmark_table.tex <==
\begin{tabularx}{1\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\raggedright\arraybackslash}X
  | >{\raggedright\arraybackslash}X | }
 \hline
 Methods & Description & Reference(s) \\ [0.5ex] 
 \hline
 Random Append & Randomly appends bytes to the end of malware samples & Suciu et al., 2019; Castro, Schmitt et al., 2019 \\ 
 \hline
 Benign Append & Appends sections of bytes from benign files to the end of malware samples & Castro, Biggio et al., 2019 \\ 
 \hline
 Enhanced Random Append & Appends better sequences that lower the confidence score the most (is not fully black box) & Chen B. et al., 2019 \\ 
 \hline
\end{tabularx}

==> experiment_3_overview.tex <==
\begin{tabularx}{1\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\raggedright\arraybackslash}X | }
 \hline
 Experiment No. & Target Anti-Malware \\ [0.5ex] 
 \hline
 Experiment \#3-1 & Malconv \\ 
 \hline
 Experiment \#3-2 & NonNeg \\ 
 \hline
 Experiment \#3-3 & ConvNet \\ 
 \hline
 Experiment \#3-4 & All three anti-malware engines (simultaneously) \\ 
 \hline
\end{tabularx}

==> experiment_3_results.tex <==
\begin{table*}[t]

\small
\caption{Comparing \malrnn's performance on three renowned DL-based anti-malware detectors with black-box AME benchmark methods across eight malware categories}
\begin{center}
\begin{tabularx}{1\textwidth} {
  | >{\centering\arraybackslash}p{1.1cm} 
  | >{\centering\arraybackslash}p{1.1cm} 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}p{1.3cm} 
  | >{\centering\arraybackslash}p{0.9cm} 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}p{0.8cm} 
  | >{\centering\arraybackslash}p{0.85cm}  |}
 \hline
 \textbf{Detector} & \textbf{Method} & \textbf{Adware} & \textbf{Backdoor} & \textbf{Botnet} & \textbf{Dropper} & \textbf{Ransomware} & \textbf{Rootkit} & \textbf{Spyware} & \textbf{Virus} & \textbf{Average} \\
 \hline
 
 \multirow{3}{*}{\textbf{Malconv}} & RA & 14.34\% & 9.88\% & 8.56\% & 14.16\% & 11.78\% & 13.21\% & 10.16\% & 11.53\% & 12.29\% \\ \cline{2-11}
 & BA & 49.15\% & 41.30\% & 20.34\% & 41.92\% & 38.44\% & 11.32\% & 35.31\% & 28.22\% & 39.43\% \\ \cline{2-11}
 & EBA & \textbf{75.55\%} & 68.29\% & 46.58\% & 69.69\% & \textbf{80.22\%} & 56.60\% & 65.31\% & 61.76\% & 69.54\% \\ \cline{2-11}
 & \textbf{MalRNN} & 68.75\% & \textbf{72.72}\% & \textbf{53.66}\% & \textbf{90\%} & 64.28\% & \textbf{69.23\%} & \textbf{80\%} & \textbf{85.71\%} & \textbf{73.24\%} \\ \cline{2-11}
 \hline
 
 \multirow{3}{*}{\textbf{NonNeg}} & RA & 0.67\% & 0.44\% & 0.19\% & 1.00\% & 0.44\% & 5.66\% & 0.63\% & 0.76\% & 0.67\% \\ \cline{2-11}
 & BA & 96.61\% & 99.41\% & 99.05\% & 94.91\% & 99.00\% & 90.57\% & 93.91\% & 88.47\% & 96.04\% \\ \cline{2-11}
 & EBA & 96.10\% & 94.40\% & 95.25\% & 98.78\% & 96.56\% & \textbf{100\%} & 94.38\% & 89.38\% & 95.45\% \\ \cline{2-11}
 & \textbf{MalRNN} & \textbf{99.87\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{99.87\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{99.97\%} \\ \cline{2-11}
 \hline
 
 \multirow{3}{*}{\textbf{ConvNet}} & RA & 30.71\% & 25.96\% & 69.01\% & 26.77\% & 10.67\% & 16.98\% & 46.88\% & 54.17\% & 33.95\% \\ \cline{2-11}
 & BA & 33.23\% & 27.43\% & 66.16\% & 35.62\% & 17.67\% & 35.85\% & 47.03\% & 49.92\% & 36.64\% \\ \cline{2-11}
 & EBA & 38.46\% & 35.29\% & 43.75\% & 47.83\% & 24.00\% & 45.28\% & 46.3\% & 51.22\% & 40.03\% \\ \cline{2-11}
 & \textbf{MalRNN} & \textbf{76.49\%} & \textbf{100\%} & \textbf{87.1\%} & \textbf{69.23\%} & \textbf{35.56\%} & \textbf{64.15\%} & \textbf{73.8\%} & \textbf{70.59\%} & \textbf{72.03\%} \\ \cline{2-11}
 \hline
 
 \multirow{3}{*}{\textbf{All Three}} & RA & 0.00\% & 0.00\% & 0.00\% & 0.55\% & 0.00\% & 1.89\% & 0.00\% & 0.00\% & 1.49\% \\ \cline{2-11}
 & BA & 15.56\% & 14.31\% & 5.30\% & 5.63\% & 9.33\% & 5.66\% & 3.75\% & 0.00\% & 8.51\% \\ \cline{2-11}
 & EBA & 23.52\% & 23.15\% & 20.53\% & 19.58\% & 23.44\% & 15.09\% & 34.69\% & 22.91\% & 22.86\% \\ \cline{2-11}
 & \textbf{MalRNN} & \textbf{34.77\%} & \textbf{54.28\%} & \textbf{23.57\%} & \textbf{46.57\%} & \textbf{29.33\%} & \textbf{41.51\%} & \textbf{45.47\%} & \textbf{34.75\%} & \textbf{38.78\%} \\ 
 \hline
\end{tabularx}
\end{center}
\label{experiment_results}
\end{table*}

==> model_parameter.tex <==
\begin{table}[H]
    \caption{MalRNN Specifications}
    \small
    \begin{tabularx}{1\textwidth} { 
      | >{\centering\arraybackslash}p{0.05\textwidth} 
      | >{\centering\arraybackslash}p{0.071\textwidth} 
      | >{\centering\arraybackslash}p{0.033\textwidth}
      | >{\centering\arraybackslash}p{0.066\textwidth} 
      | >{\centering\arraybackslash}p{0.13\textwidth}
      | >{\centering\arraybackslash}p{0.07\textwidth} |}
     \cline{1-6}
     \multicolumn{2}{|c|}{\textbf{Layer}} & \textbf{\# of Units} & \textbf{Activation Type} & \textbf{Output Shape} & \textbf{Layer-specific} \\ 
     \cline{1-6}
     \multirow{2}{*}{Encoder} & Embedding & 256 & - & (B-size, 256, 100) & Vocabulary size=256 \\
     \cline{2-6}
      & GRU & 100 & Tanh & (B-size, 100, 100) & Initial bias=0 \\
     \cline{1-6}
     \multirow{2}{*}{Decoder} & GRU & 100 & Tanh & (B-size, 100, 100) & Initial bias=0 \\
     \cline{2-6}
      & Fully Connected Layer & 128 & Softmax & (B-size, 100, 256) & Initial bias=0 \\
     \cline{1-6}
     \multicolumn{6}{|l|}{Learning Rate=0.01, B-size (Batch size)=10, Systematic sampling rate=$10^{-3}$,}\\
     \multicolumn{6}{|l|}{Maximum number of attempts: 50, Maximum append size: 40\%.}\\
     \cline{1-6}
    \end{tabularx}
\label{model_parameters}
\end{table}

==> test.tex <==
\begin{table}[]
    \small
    \begin{tabularx}{0.6\textwidth} { 
      | >{\raggedright\arraybackslash}p{1.5cm}
      | >{\raggedright\arraybackslash}p{1.25cm}
      | >{\raggedright\arraybackslash}p{1.5cm}
      | >{\raggedright\arraybackslash}X 
      | >{\raggedright\arraybackslash}X | }
     \hline
     \textbf{Layer} & \textbf{Number of Units} & \textbf{Activation Type} & \textbf{Output Shape} & \textbf{Layer-specific parameters} \\ [0.5ex] 
     \hline
     Embedding & 256 & - & (Batch\_size, 256, 100) & Vocabulary\_ size = 256 \\
     \hline
     GRU & 100 & Tanh & (Batch\_size, 100, 100) & Bias\_initializer= 0 \\
     \hline
     Fully Connected Layer & 128 & Softmax & (Batch\_size, 100, 256) & Bias\_initializer= 0 \\
     \hline
     \multicolumn{5}{|l|}{Learning Rate = 0.01, Batch\_size = 10, Systematic Sampling Rate: $10^{-4}$}\\
     \hline
    \end{tabularx}
\end{table}

==> testbed_table.tex <==
\begin{table}[ht]
\small
\caption{Breakdown of testbed based on different malware categories}
\begin{tabularx}{0.5\textwidth} { 
  | >{\centering\arraybackslash}X
  | >{\centering\arraybackslash}p{3cm}  
  | >{\centering\arraybackslash}X   | }
 \hline
 \textbf{Malware Category} & \textbf{Examples} & \textbf{\# of Malware Samples} \\ [0.5ex] 
 \hline
 Adware & eldorado, razy, gator & 1,947\\
 \hline
 Backdoor & lunam, rahack, symmi & 678\\
 \hline
 Botnet & virut, salicode, sality & 526 \\ 
 \hline
 Dropper & dunwod, gepys, doboc & 904\\
 \hline
 Ransomware & vtflooder, msil, bitman & 900\\
 \hline
 Rootkit & onjar, dqqd, shipup & 53\\
 \hline
 Spyware & mikey, qqpass, scar & 640 \\
 \hline
 Virus & nimda, shodi, hematite & 659\\
 \hline
 Total & All subtypes & 6,307\\
 \hline
\end{tabularx}
\label{testbed}
\end{table}
